Probing Linguistic Information For Logical Inference In Pre-trained Language Models

Progress in pre-trained language models has led to a surge of impressive results on downstream tasks for natural language understanding. Recent work on probing pre-trained language models uncovered a wide range of linguistic properties encoded in their contextualized representations. However, it is unclear whether they encode semantic knowledge that is crucial to symbolic inference methods. We propose a methodology for probing linguistic information for logical inference in pre-trained language model representations. Our probing datasets cover a list of linguistic phenomena required by major symbolic inference systems. We find that (i) pre-trained language models do encode several types of linguistic information for inference, but there are also some types of information that are weakly encoded, (ii) language models can effectively learn missing linguistic information through fine-tuning. Overall, our findings provide insights into which aspects of linguistic information for logical inference do language models and their pre-training procedures capture. Moreover, we have demonstrated language models' potential as semantic and background knowledge bases for supporting symbolic inference methods.

==> probing linguistic information arxiv/graph.tex <==
\newcommand{\sem}[1]{[\![ #1 ]\!]}
\newcommand{\stringFont}[1]{\texttt{#1}}
\newcommand{\strcat}[1]{\ensuremath{\stringFont{#1}}}
\newcommand{\symb}{\ensuremath{\mathbf{sym}}}
\newcommand{\brcat}[2]{\ensuremath{(_{#2}\,\strcat{#1})}}

\newcommand{\catFont}[1]{\textsc{#1}}
\newcommand{\catS}{\textsc{S}}
\newcommand{\catPN}{\textsc{PN}}
\newcommand{\catNP}{\textsc{NP}}
\newcommand{\catVP}{\textsc{VP}}
\newcommand{\catVNEG}{\ensuremath{\catFont{Vneg}}}
\newcommand{\catVPpast}{\ensuremath{\catFont{VP}_{\text{past}}}}
\newcommand{\catVPbase}{\ensuremath{\catFont{VP}_{\text{base}}}}
\newcommand{\catIV}{\textsc{IV}}
\newcommand{\catIVdash}{\textsc{IV}$'$}
\newcommand{\catTV}{\textsc{TV}}
\newcommand{\catQ}{\textsc{Q}}
\newcommand{\catN}{\textsc{N}}
\newcommand{\catNhyp}{\textsc{N}$_{\text{hyp}}$}
\newcommand{\WhNP}{\textrm{WhNP}}
\newcommand{\catAdj}{\textsc{Adj}}
\newcommand{\catAdv}{\textsc{Adv}}
\newcommand{\catPP}{\textsc{PP}}
\newcommand{\relC}{\textsc{RelC}}
\newcommand{\catSbar}{\ensuremath{\overline{\mbox{\textsc{S}}}}}
\newcommand{\midspace}{\ensuremath{\ \mid \ }}
\newcommand{\LF}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\drgvar}[1]{\texttt{\textbf{#1}}}
\newcommand{\righte}{$G\Rightarrow P$}
\newcommand{\lefte}{$G\Leftarrow P$}
\newcommand{\bie}{$G\Leftrightarrow P$}
\newcommand{\modelcite}[1]{\citeauthor{#1},\ \citeyear{#1}}

\newcommand{\PredRepl}[1]{\underline{#1}}
\newcommand{\PredReplColor}[1]{\orangebox{#1}}
\newcommand{\Qf}[1]{\underline{#1}}
\newcommand{\QfColor}[1]{\greenbox{#1}}
\newcommand{\ClColora}[1]{\blueboxa{#1}}
\newcommand{\ClColorb}[1]{\blueboxb{#1}}
\newcommand{\Repl}[1]{\textsc{#1}}

\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\newcommand{\ModifierColor}[1]{\redbox{#1}}
\newcommand{\QuantifierColor}[1]{\bluebox{#1}}
\newcommand{\NegationColor}[1]{\greenbox{#1}}


\definecolor{olive} {cmyk} {0.64, 0.00, 0.95, 0.40}
\newcommand{\corr}[1]{\hspace{3em}\textcolor{olive}{#1}}
\newcommand{\wrong}[1]{\hspace{3em}\textcolor{red}{#1}}

\newcommand{\pospol}[1]{#1\ensuremath{^{\textcolor{red}{\uparrow}}}}
\newcommand{\negpol}[1]{#1\ensuremath{^{\textcolor{blue}{\downarrow}}}}
\newcommand{\setof}[1]{\ensuremath{\left \{ #1 \right \}}}

%%%%%%%% MyBox %%%%%%%%%%%%%%
\usepackage{tcolorbox}
\newtcbox{\redbox}{on line,
  colframe=red,colback=red!5!white,
%  sharp corners,
  boxrule=0.3mm,
  arc=0.5mm,
  boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt
  }

\newtcbox{\bluebox}{on line,
  colframe=blue,colback=blue!5!white,
%  sharp corners,
  boxrule=0.3mm,
  arc=0.5mm,
  boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt
  }

\newtcbox{\greenbox}{on line,
  colframe=applegreen,colback=applegreen!5!white,
%  sharp corners,
  boxrule=0.3mm,
  arc=0.5mm,
  boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt
  }
  
\newtcbox{\orangebox}{on line,
  colframe=orange,colback=orange!10!white,
  boxrule=0.3mm,
  arc=1.0mm,
  boxsep=0pt,left=1pt,right=1pt,top=1pt,bottom=1pt
  }

% \newtcbox{\greenbox}{on line,
%   colframe=green!70!black,colback=green!10!white,
%   boxrule=0.3mm,
%   arc=1.0mm,
%   boxsep=0pt,left=1.0pt,right=1.0pt,top=1.0pt,bottom=1.0pt
%   }
  
\newtcbox{\blueboxa}{on line,
  colframe=blue!70!black,colback=blue!5!white,
  boxrule=0.3mm,
  arc=1.0mm,
  boxsep=0pt,left=1.2pt,right=1.2pt,top=1.3pt,bottom=1.3pt
  }

\newtcbox{\blueboxb}{on line,
  colframe=blue!70!black,colback=blue!5!white,
  boxrule=0.3mm,
  arc=1.0mm,
  boxsep=0pt,left=1.2pt,right=1.2pt,top=1.6pt,bottom=1.6pt
  }

\newtcbox{\graybox}{on line,
  colframe=white,colback=gray!15!white,
  boxrule=0mm,left=1pt,right=1pt,top=1pt,bottom=1pt
  }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> probing linguistic information arxiv/settings.tex <==
\usepackage{amsmath}
\usepackage{tabularx}
\usepackage{amssymb}
%\usepackage{amsfonts}
\usepackage{arydshln}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{tikz}
\usetikzlibrary{tikzmark}


\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\newcommand{\tx}[1]{``\textit{#1}''}
\newcommand{\sptk}[1]{\texttt{[#1]}}
\newcommand{\eqform}[1]{Equation~(\ref{#1})}

% \DeclareMathOperator\softmax{\operatorname{softmax}}
% \DeclareMathOperator\softsign{\operatorname{softsign}}
% \DeclareMathOperator\sigm{\operatorname{sigm}}
% \DeclareMathOperator\sigmoid{\operatorname{sigmoid}}
% \DeclareMathOperator\mytanh{\operatorname{tanh}}
% \DeclareMathOperator\avg{\operatorname{avg}}
% \DeclareMathOperator\var{\operatorname{var}}
% \DeclareMathOperator\minimize{\operatorname{minimize}}
% \DeclareMathOperator\maximize{\operatorname{maximize}}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\mlp}{\operatorname{MLP}}
% \DeclareMathOperator*{\lstm}{\operatorname{f_{LSTM}}}

%\usepackage{algorithm}
%\usepackage[noend]{algpseudocode}

\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{officeblue}{RGB}{0,102,204}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}
\definecolor{mylightgreen}{rgb}{0,128,0}
\definecolor{mybrickred}{RGB}{182,50,28}
\newcommand\mybox[2][]{\tikz[overlay]\node[inner sep=1pt, anchor=text, rectangle, rounded corners=1mm,#1] {#2};\phantom{#2}}
\definecolor{fillcolor}{RGB}{216,217,252}
\newcommand\bg[1]{\mybox[fill=blue!20]{#1}}
\newcommand\rg[1]{\mybox[fill=red!20]{#1}}

\definecolor{bblue}{HTML}{ADD8E6}
\definecolor{yyellow}{HTML}{FFFF00}
\definecolor{rred}{HTML}{FF6361}
\definecolor{ppink}{HTML}{BC5090}
\definecolor{ppurple}{HTML}{58508D}

\DeclareRobustCommand{\hlyellow}[1]{{\sethlcolor{yyellow}\hl{#1}}}
\DeclareRobustCommand{\hlblue}[1]{{\sethlcolor{bblue}\hl{#1}}}

%%%%%Algorithm Box Package%%%%%
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\algnewcommand\algorithmicrequireb{{\hspace{0.85cm}}}
%\algnewcommand\INPTDESCB{\item[\algorithmicrequireb]}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\algnewcommand\algorithmicfuncdesc{\textbf{Function:}}
%\algnewcommand\FUNCDESC{\item[\algorithmicfuncdesc]}
%\algnewcommand\algorithmicfuncdescb{{\hspace{1.48cm}}}
%\algnewcommand\FUNCDESCB{\item[\algorithmicfuncdescb]}
%\algnewcommand{\algorithmicgoto}{\textbf{goto}}
%\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}
%\newcommand*\Let[2]{\State {#1 $\gets$ #2}}
%\newcommand*\LineLet[2]{#1 $\gets$ #2}
%\newcommand*\AddOne[1]{\State #1 $\gets$ #1 $+1$}
%\newcommand*\AddOne[1]{\State #1 $++$}
%\newcommand*\LineComment[1]{\Statex \(\triangleright\) #1}
%\newcommand*\LineFor[2]{\State {\algorithmicfor~#1~\algorithmicdo~~~~#2}}
%\newcommand*\LineIf[2]{\State {\algorithmicif~#1~\algorithmicthen~~~~#2}}
%\newcommand*\AlgCommentInLine[1]{{\color{deepblue}{$\triangleright$ \textit{#1}}}}
%\newcommand*\AlgComment[1]{\State{\AlgCommentInLine{#1}}}
%%%%%Algorithm Box Package%%%%%

\newcommand\mycode[1]{\textsf{\fontsize{10}{12}\selectfont #1}}


==> probing linguistic information arxiv/tables/data_example.tex <==
\begin{table*}[t!]
    \centering
    \small
    \scalebox{0.75}{\begin{tabular}{l l l}  \toprule %
    
    \textbf{Task} & \textbf{Probe Type} & \textbf{Example} \\\midrule
     
    Semantic-Graph & edge probing & A \ModifierColor{tall} \NegationColor{boy} is \QuantifierColor{running} \ModifierColor{quickly} to catch a \ModifierColor{soccer} \NegationColor{ball}. \\[5pt]
    
    (SemGraph) & & \NegationColor{[boy]} \QuantifierColor{[running]}  $\longrightarrow$ \textbf{Concept-Relation}; \ModifierColor{[tall]} \NegationColor{[boy]} $\longrightarrow$ \textbf{Concept-Modifier};\\[5pt] 
    
    & & \ModifierColor{[quickly]} \QuantifierColor{[running]} $\longrightarrow$ \textbf{Relation-Modifier} \\[5pt] \midrule
    
    Monotonicity & vertex probing & Some$^\uparrow$ people$^\uparrow$ in$^\uparrow$ the$^\uparrow$ White$^=$ House$^=$ does$^\uparrow$ not$^\uparrow$ know$^\downarrow$ if$^\downarrow$ any$^\downarrow$ dog$^\downarrow$ in$^\downarrow$ Ohio$^\downarrow$ ate$^\downarrow$ bananas$^\downarrow$ yesterday$^\downarrow$ \\[5pt] \midrule
    
    Lexical & edge probing & P: The \QuantifierColor{[man]$_{s^1}$} is holding a \ModifierColor{[saxophone]$_{s^2}$} \\[5pt]
    (SA-Lex) & & H: The man is holding an \ModifierColor{[instrument]$_{s^3}$}. \\[5pt]
    & & ($s_1$, $s_3$) $\longrightarrow$ \textbf{Unaligned}; ($s_2$, $s_3$) $\longrightarrow$ \textbf{Aligned} \\\midrule
     
    Anaphora & edge probing & The \QuantifierColor{[technician]$_{s^1}$} told the \ModifierColor{[customer]$_{s^2}$} that \ModifierColor{[he]$_{s^3}$} could pay with cash.  \\[5pt]
    (SA-AP) & & ($s_1$, $s_3$) $\longrightarrow$ \textbf{Unaligned}; ($s_2$, $s_3$) $\longrightarrow$ \textbf{Aligned} \\\midrule
    
    Sentiment & vertex probing   & P: When asked about the restaurant, Brielle said, ``\ModifierColor{[It]$_{t^1}$ [was]$_{t^2}$ [terrible!]$_{t^3}$} \\
    (SA-ST) & & \QuantifierColor{[I]$_{t^4}$ [found]$_{t^5}$ [this]$_{t^6}$ [product]$_{t^7}$ [to]$_{t^8}$ [be]$_{t^9}$ [way]$_{t^{10}}$ [too]$_{t^{11}}$ [big]$_{t^{12}}$} '' \\[5pt]
    & & H: Brielle \ModifierColor{[did]$_{t^{13}}$ [not]$_{t^{14}}$ [like]$_{t^{15}}$ [the]$_{t^{16}}$ [restaurant]$_{t^{17}}$}  \\[5pt]
    & & \{$t^1$, $\dots$, $t^3$\} $\longrightarrow$ \textbf{Align}$_1$; \{$t^4$, $\dots$, $t^{12}$\} $\longrightarrow$ \textbf{Unaligned}; \{$t^{13}$, $\dots$, $t^{17}$\} $\longrightarrow$ \textbf{Align}$_2$ \\\midrule
    
    Relational-Knowledge & vertex probing & P: \ModifierColor{[Dirk]$_{t^1}$ [Nowitski]$_{t^2}$ [is]$_{t^3}$ [a]$_{t^4}$ [current]$_{t^5}$ [NBA]$_{t^6}$ [star]$_{t^7}$} playing with the \\[5pt]
    (SA-RK) & & \;\;\; \QuantifierColor{[Dallas]$_{t^8}$ [Mavericks]$_{t^9}$ [as]$_{t^{10}}$ [an]$_{t^{11}}$ [all-purpose]$_{t^{12}}$ [forward]$_{t^{13}}$} \\[5pt]
    & & H: \ModifierColor{[Dirk]$_t^{14}$ [Nowitski]$_t^{15}$ [plays]$_t^{16}$ [in]$_t^{17}$ [the]$_t^{18}$ [NBA]$_t^{19}$} \\[5pt]
    & & \{$t^1$, $\dots$, $t^7$\} $\longrightarrow$ \textbf{Align}$_1$; \{$t^8$, $\dots$, $t^{13}$\} $\longrightarrow$ \textbf{Unaligned}; \{$t^{14}$, $\dots$, $t^{19}$\} $\longrightarrow$ \textbf{Align}$_2$ \\\midrule
    
    Contradiction Signature & vertex probing & P: Italy and Germany \QuantifierColor{[have]$_{t^1}$ [each]$_{t^2}$ [played]$_{t^3}$ [twice]$_{t^4}$}, \\[5pt]
     (ContraSig) & & \;\;\;  and they \NegationColor{[haven't]$_{t^5}$ [beaten]$_{t^6}$ [anybody]$_{t^7}$ [yet]$_{t^8}$} \\[5pt]          
     & & H: Italy \NegationColor{[defeats]$_{t^9}$ [Germany]$_{t^{10}}$} \\[5pt]
     & & \{$t^1$, $\dots$, $t^4$\} $\longrightarrow$ \textbf{None}$_1$; \{$t^5$, $\dots$, $t^8$\} $\longrightarrow$ \textbf{Contra-sig}$_1$; \{$t^9$, $t^{10}$\} $\longrightarrow$ \textbf{Contra-sig}$_2$ \\
      
      \bottomrule
      \end{tabular}}
    \caption{\small This table lists examples of our probing tasks. For semantic graph construction task, the red, green and blue boxes denote modifiers, concepts and relations respectively. For semantic alignment tasks and the contradiction signature detection task, the red boxes are spans that are semantically aligned. The green boxes are spans that form a contradiction signature. The blue boxes are spans that are irrelevant to semantic alignment or contradiction. Here P stands for a premise, and H stands for a hypothesis. The anaphora-based alignment only uses a single sentence. For the labels, ($s^1, s^3$) $\longrightarrow$ \textbf{Aligned} means that $s^1$ and $s^3$ are aligned. \{$t^1$, $\dots$, $t^7$\} $\longrightarrow$ \textbf{Align}$_1$ means that tokens $t^1$ to $t^7$ belongs to the first phrase in a semantically aligned pair.}
    \label{tab:data_exp}
\end{table*}

==> probing linguistic information arxiv/tables/dataset.tex <==
\begin{table}[t!]
    \centering
    \footnotesize
    \scalebox{0.80}{
    \begin{tabular}{l l r r}
        \toprule
        \textbf{Task} & \textbf{Split} & \textbf{\# S} & \textbf{Origin}  \\\midrule
        
        \multirow{2}{*}{\textbf{SemGraph}}
        & train & 10,000 & \cite{bowman-etal-2015-large}        \\     
        & test & 5,000   & \cite{bowman-etal-2015-large}         \\ \hline
        
        \multirow{2}{*}{\textbf{ContraSig}}
        & train & 1,000 & \cite{Marelli2014ASC}                 \\     
        & test & 500    & \cite{Marelli2014ASC}           \\ \hline
        
        \multirow{2}{*}{\textbf{Monotonicity}}
        & train & 5,000 & \cite{yanaka-etal-2019-neural}        \\     
        & test & 500    & \cite{chen-gao-2021-IWCS}               \\ \hline
        
        \multirow{2}{*}{\textbf{SA-Lex}}
        & train & 1,000 & \cite{glockner-etal-2018-breaking}    \\     
        & test & 500    & \cite{glockner-etal-2018-breaking}      \\ \hline
        
        \multirow{2}{*}{\textbf{SA-ST}}
        & train & 1,000 & \cite{poliak-etal-2018-collecting}    \\     
        & test & 600    & \cite{poliak-etal-2018-collecting}      \\ \hline
        
        \multirow{2}{*}{\textbf{SA-AP}}
        & train & 500 & \cite{rudinger-etal-2018-gender}        \\     
        & test & 220  & \cite{rudinger-etal-2018-gender}        \\ \hline
        
        \multirow{2}{*}{\textbf{SA-RK}}
        & train & 1,000 & \cite{poliak-etal-2018-collecting}    \\     
        & test & 500    & \cite{poliak-etal-2018-collecting}      \\
        
        \bottomrule
    \end{tabular}}
    
    \caption{ \small This table shows dataset details for each probing task. We list the number of training and testing examples, and also the datasets that the train and test sets are recast from.}
    \label{tab:data_detail}
\end{table}

==> probing linguistic information arxiv/tables/finetune.tex <==
%% INSTANCE-LEVEL ACCURACY

\begin{table}[t!]
    \centering
    \footnotesize
    \scalebox{0.8}{
    \begin{tabular}{l c c c}
        \toprule
            \textbf{Model} & \textbf{Monotonicity} &\textbf{SA-ST} & \textbf{SA-RK} \\
        \hline 
        
        %\multicolumn{9}{c}{Group 4: \textbf{Language Models} (best probings on fine-tuned NLI models, \textbf{accuracy gains} are shown in parenthesis)} \\ 
        \textbf{BERT}-base  & 60.9 ({\large \color{cyan} $\blacktriangle$} 2.8) & 79.8 ({\large \color{cyan} $\blacktriangle$} 12.7) & 81.4 ({\large \color{cyan} $\blacktriangle$} 14.2) \\
       
        \textbf{BERT}-large & 60.2 ({\large \color{cyan} $\blacktriangle$} 2.8) & 77.6 ({\large \color{cyan} $\blacktriangle$} 10.2) & 80.5 ({\large \color{cyan} $\blacktriangle$} 14.6) \\
        
        \cdashline{1-4}
        
        \textbf{RoBERTa}-base   
        & 59.4 ({\large \color{cyan} $\blacktriangle$} 9.3) & 78.0 ({\large \color{cyan} $\blacktriangle$} 11.9) & 88.0 ({\large \color{cyan} $\blacktriangle$} 22.7) \\
        
        \textbf{RoBERTa}-large 
        & 58.0 ({\large \color{cyan} $\blacktriangle$} 2.6) & 76.1 ({\large \color{cyan} $\blacktriangle$} 10.4) & 89.7 ({\large \color{cyan} $\blacktriangle$} 27.7) \\
        
        \cdashline{1-4}
        
        \textbf{DeBERTa}        
        & 68.7 ({\large \color{cyan} $\blacktriangle$} 3.0) & 78.9 ({\large \color{cyan} $\blacktriangle$} 14.9) & 89.6 ({\large \color{cyan} $\blacktriangle$} 19.1) \\
        
        \bottomrule 
    \end{tabular}}
    
    \caption{\small Probing accuracy (\%) of fine-tuned NLI models on probing tasks that did not benefit from pre-trained models.}
    \label{tab:finetune}
\end{table}

==> probing linguistic information arxiv/tables/information_gain.tex <==
%% INSTANCE-LEVEL ACCURACY

\begin{table}[t!]
    \centering
    \footnotesize
    \scalebox{0.75}{
    \begin{tabular}{l l l l l}
    
    \toprule
    \textbf{Model} & \textbf{SemGraph} & \textbf{ContraSig} & \textbf{Monotonicity} & \textbf{SA-Lex} \\ \hline 
 
        %\multicolumn{9}{c}{Group 2: \textbf{Language Models} (\textbf{MLP} classifier probing, no fine-tuning} \\
        \textbf{BERT}-base      
        & 0.10 (6\%) & 1.16 (65\%) & 0.82 (58\%) & 1.16 (116\%) \\
        
        \textbf{BERT}-large     
        & 0.08 (5\%) & 1.15 (64\%) & 0.8 (56\%) & 1.14 (114\%) \\
        
        \cdashline{1-5}
        
        \textbf{RoBERTa}-base   
        & 0.10 (6\%) & 1.16 (65\%) & 0.85 (60\%) & 1.14 (114\%) \\
        
        \textbf{RoBERTa}-large  
        & 0.09 (5\%) & 1.14 (64\%) & 0.9 (63\%) & 1.15 (115\%) \\
        
        \cdashline{1-5}
        
        \textbf{DeBERTa}       
        & 0.11 (7\%) & 1.16 (65\%) & 0.78 (55\%) & 1.16 (116\%) \\ 
        
        \hline
    
    & \textbf{SA-ST} & \textbf{SA-AP} & \textbf{SA-RK} & \textbf{Avg} \\ \hline
    
        \textbf{BERT}-base      
        & 0.39 (39\%) & 1.07 (54\%) & 0.74 (80\%) & 0.78 (59\%) \\
        
        \textbf{BERT}-large     
        & 0.41 (41\%) & 1.02 (51\%) & 0.74 (80\%) & 0.76 (59\%) \\
        
        \cdashline{1-5}
        
        \textbf{RoBERTa}-base   
        & 0.74 (74\%) & 1.04 (52\%) & 0.80 (86\%) & 0.83 (65\%) \\
        
        \textbf{RoBERTa}-large  
        & 0.62 (62\%) & 1.05 (53\%) & 0.78 (84\%) & 0.82 (64\%) \\
        
        \cdashline{1-5}
        
        \textbf{DeBERTa}       
        & 0.67 (67\%) & 1.02 (51\%) & 0.67 (72\%) & 0.79 (62\%) \\ 

    \bottomrule 
    \end{tabular}}
    
    \caption{\small Results on infromation-theoretic probing. Here we show the amount of extra information each language model shares, compared to the best baseline word embedding. The percentage of information gain is listed in the parenthesis.}
    \label{tab:information_gain}
\end{table}

==> probing linguistic information arxiv/tables/instance_accuracy.tex <==
%% INSTANCE-LEVEL ACCURACY

\begin{table*}[t!]
    \centering
    \footnotesize
    \scalebox{0.85}{
    \begin{tabular}{l c c c c c c c c}
        \toprule
            \textbf{Model} & \textbf{SemGraph} & \textbf{ContraSig} & \textbf{Monotonicity} & \textbf{SA-Lex} & \textbf{SA-ST} & \textbf{SA-AP} & \textbf{SA-RK} \\
        \hline 
        
        \multicolumn{9}{c}{Group 1: \textbf{Baselines} (direct probing, no fine-tuning)} \\ \hline 
        \textbf{Random}     & 68.5 & 29.7 & 48.8 & 45.5 & 46.8 & 48.9 & 45.7 \\
        \textbf{Word2Vec}   & 68.8 & 42.4 & 43.4 & 59.7 & 31.4 & 32.3 & 42.3 \\
        \textbf{Glove}      & 71.3 & 40.2 & 41.3 & 60.6 & 33.4 & 35.8 & 50.5 \\
        \textbf{FastText}   & 69.4 & 31.7 & 51.9 & 50.1 & 51.3 & 51.3 & 52.2 \\
        \hline
 
        \multicolumn{9}{c}{Group 2: \textbf{Language Models} (\textbf{Linear} classifier probing, no fine-tuning; \textbf{selectivity} is shown in parenthesis)} \\ \hline
        \textbf{BERT}-base      & 91.8 (42.0) & 58.5 (35.1) & 48.5 (35.8) & 57.4 (7.30) &  56.3 (34.7) & 49.8 (0.1) &  62.8 (50.3) \\
        \textbf{BERT}-large     & 88.9 (39.5) & 51.6 (37.9) & 44.9 (37.4) & 55.5 (4.80) &  51.2 (33.1) & 50.2 (0.1) &  62.1 (49.5) \\
        \cdashline{1-9}
        \textbf{RoBERTa}-base   & 88.9 (39.2) & 52.2 (33.0) & 42.8 (42.3) & 61.4 (11.3) &  47.5 (38.6) & 49.4 (0.6) & 62.3 (49.7) \\
        \textbf{RoBERTa}-large  & 89.6 (40.0) & 48.4 (27.6) & 38.1 (43.0) & 66.2 (16.2) &  46.1 (36.6) & 49.8 (0.3) & 62.9 (50.1) \\
        \cdashline{1-9}
        \textbf{DeBERTa}        & \textbf{93.4} (43.7) & 78.5 (32.3) & 54.9 (42.2) & 83.8 (33.2) &  42.8 (35.7) & 51.8 (2.3) & 65.6 (52.8) \\
        \hline
        
        \multicolumn{9}{c}{Group 3: \textbf{Language Models} (\textbf{MLP} classifier probing, no fine-tuning; \textbf{selectivity} is shown in parenthesis)} \\ \hline
        \textbf{BERT}-base      & 90.7 (40.7) & 91.6 (31.7) & 58.1 (41.3) & 89.0 (38.8) &  67.1 (34.3) & 61.5 (17.6) & 70.9 (54.7) \\
        \textbf{BERT}-large     & 89.3 (38.0) & 91.0 (33.0) & 57.4 (34.6) & 88.8 (38.4) &  \textbf{67.4} (35.5) & 77.6 (31.3) & 69.0 (53.1) \\
        \cdashline{1-9}
        \textbf{RoBERTa}-base   & 91.5 (39.5) & 92.5 (27.8) & 50.1 (49.1) & 87.2 (36.6) &  66.1 (37.3) & 87.0 (38.6) & 70.9 (52.9) \\
        \textbf{RoBERTa}-large  & 90.1 (40.6) & 91.9 (35.5) & 55.4 (46.8) & 88.9 (37.2) &  65.7 (38.2) & \textbf{88.6} (39.3) & 70.2 (49.1) \\
        \cdashline{1-9}
        \textbf{DeBERTa}        & 92.3 (42.2) & \textbf{92.9} (32.5) & \textbf{65.7} (58.6) & \textbf{91.0} (41.5) &  63.0 (36.9) & 85.2 (37.3) & \textbf{72.9} (58.2) \\
        
        \bottomrule 
    \end{tabular}}
    
    \caption{\small This table lists results from the probing and fine-tuning experiments We include in group 1 probing accuracy (\%) from two baselines. Group 2 and 3 shows probing accuracy (\%) of the linear classifier (group 2) and the MLP classifier (group 3). For each probe, we also record the selectivity score (\%) from control tasks.}
    \label{tab:instance}
\end{table*}

==> probing linguistic information arxiv/tables/plots.tex <==
\begin{figure}[t!]
    \centering
     \begin{subfigure}[t]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/relational_vertex_label.pdf}
         \label{fig:contra_label}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[t]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/sentiment_vertex_label.pdf}
         \label{fig:mono_label}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[t]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/lexical_label.pdf}
     \end{subfigure}
     \label{fig:lex_label}\\
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/anaphora_label.pdf}
         \label{fig:contra_label}
     \end{subfigure}
     \bigskip
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/contradict_vertex_label.pdf}
         \label{fig:rk_label}
     \end{subfigure} \\
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/monotonicity_label.pdf}
         \label{fig:st_label}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/semgraph2_label.pdf}
         \label{fig:st_label}
     \end{subfigure}
     
     \caption{\small Plots here shows label-wise accuracy across models for each inference information probing task. Here LM1-5 stands for the five language models in order (BERT-base, BERT-large, RoBERTa-base, RoBERTa-large, DeBERTa).}
     \label{fig:acc_label}
\end{figure}

==> probing linguistic information arxiv/tables/task_example.tex <==
\begin{table*}[t!]
    \centering
    \small
    
    \scalebox{0.85}{\begin{tabular}{l l}  \toprule %
    
    \textbf{Task} & \textbf{Example} \\\midrule
     
    Semantic-Graph & A \ModifierColor{tall} \NegationColor{boy} is \QuantifierColor{running} \ModifierColor{quickly} to catch a \ModifierColor{soccer} \NegationColor{ball}. \\[5pt]
    (SemGraph) & \NegationColor{[boy]} \QuantifierColor{[running]}  $\longrightarrow$ \textbf{Concept-Relation}; \ModifierColor{[tall]} \NegationColor{[boy]} $\longrightarrow$ \textbf{Concept-Modifier};\\[5pt] 
    & \ModifierColor{[quickly]} \QuantifierColor{[running]} $\longrightarrow$ \textbf{Relation-Modifier} \\[5pt] \midrule
    
    Monotonicity & Some$^\uparrow$ people$^\uparrow$ in$^\uparrow$ the$^\uparrow$ White$^=$ House$^=$ does$^\uparrow$ not$^\uparrow$ know$^\downarrow$ if$^\downarrow$ any$^\downarrow$ dog$^\downarrow$ in$^\downarrow$ Ohio$^\downarrow$ ate$^\downarrow$ bananas$^\downarrow$ yesterday$^\downarrow$ \\ \midrule
    
    Lexical & P: The \QuantifierColor{man} is holding a \ModifierColor{saxophone} \\ [5pt]
    (SA-Lex) & H: The man is holding an \ModifierColor{instrument}. \\ [5pt]
    & \QuantifierColor{[man]} \ModifierColor{[instrument]}  $\longrightarrow$ \textbf{Unaligned}; \ModifierColor{[saxophone]} \ModifierColor{[instrument]} $\longrightarrow$ \textbf{Aligned} \\ [5pt] \midrule
     
    Anaphora & The \QuantifierColor{technician} told the \ModifierColor{customer} that \ModifierColor{he} could pay with cash.  \\[5pt]
    (SA-AP) & \QuantifierColor{[technician]} \ModifierColor{[he]}  $\longrightarrow$ \textbf{Unaligned}; \ModifierColor{[customer]} \ModifierColor{[he]} $\longrightarrow$ \textbf{Aligned} \\ [5pt] \midrule
    
    Sentiment & P: When asked about the restaurant, Brielle said, ``\ModifierColor{It was terrible!} \QuantifierColor{I found this product to be way too big} '' \\[5pt]
    (SA-ST) & H: Brielle \ModifierColor{did not like the restaurant}  \\[5pt]
    & \QuantifierColor{[I found this product to be way too big]} \ModifierColor{[did not like the restaurant]} $\longrightarrow$ \textbf{Unaligned}\\  [5pt] 
    & \ModifierColor{[It was terrible]} \ModifierColor{[did not like the restaurant]} $\longrightarrow$ \textbf{Aligned} \\ [5pt] \midrule
    
    Relational-Knowledge & P: \ModifierColor{Dirk Nowitski is a current NBA star} playing with the \QuantifierColor{Dallas Mavericks as an all-purpose forward} \\[5pt]
    (SA-RK) & H: \ModifierColor{Dirk Nowitski plays in the NBA} \\[5pt] 
    & \QuantifierColor{[Dallas Mavericks as an all-purpose forward]} \ModifierColor{[Dirk Nowitski plays in the NBA]} $\longrightarrow$ \textbf{Unaligned} \\ [5pt] 
    & \ModifierColor{[Dirk Nowitski is a current NBA star]} \ModifierColor{[Dirk Nowitski plays in the NBA]} $\longrightarrow$ \textbf{Aligned} \\ [5pt]  \midrule
    
    Contradiction Signature & P: Italy and Germany \QuantifierColor{have each played twice}, and they \NegationColor{haven't beaten anybody yet} \\[5pt]
     (ContraSig) & H: Italy \NegationColor{defeats Germany} \\[5pt]
     & \QuantifierColor{[have each played twice]} \NegationColor{[defeats Germany]} $\longrightarrow$ \textbf{None} \\ [5pt] 
     & \NegationColor{[haven't beaten anybody yet]} \NegationColor{[defeats Germany]} $\longrightarrow$ \textbf{Contra-sig} \\ [5pt] 
      
      \bottomrule
      \end{tabular}}
      \caption{\small This table lists examples for the semantic alignment tasks and the contradiction signature detection task. The red boxes are spans that are semantically aligned. The yellow boxes are spans that form a contradiction signature. The blue boxes are spans that are irrelevant to semantic alignment or contradiction. Here P stands for a premise, and H stands for a hypothesis. The anaphora-based alignment only uses a single sentence. For the labels, ($s^1, s^3$) $\longrightarrow$ \textbf{Aligned} means that $s^1$ and $s^3$ are aligned. \{$t^1$, $\dots$, $t^7$\} $\longrightarrow$ \textbf{Align}$_1$ means that tokens $t^1$ to $t^7$ belongs to the first phrase in a semantically aligned pair.}
    \label{tab:data_exp}
\end{table*}

==> tables/plots.tex <==
\begin{figure}[t!]
    \centering
     \begin{subfigure}[t]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/relational_vertex_label.pdf}
         \label{fig:contra_label}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[t]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/sentiment_vertex_label.pdf}
         \label{fig:mono_label}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[t]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/lexical_label.pdf}
     \end{subfigure}
     \label{fig:lex_label}\\
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/anaphora_label.pdf}
         \label{fig:contra_label}
     \end{subfigure}
     \bigskip
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/contradict_vertex_label.pdf}
         \label{fig:rk_label}
     \end{subfigure} \\
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/monotonicity_label.pdf}
         \label{fig:st_label}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/semgraph2_label.pdf}
         \label{fig:st_label}
     \end{subfigure}
     
     \caption{\small Plots here shows label-wise accuracy across models for each inference information probing task. Here LM1-5 stands for the five language models in order (BERT-base, BERT-large, RoBERTa-base, RoBERTa-large, DeBERTa).}
     \label{fig:acc_label}
\end{figure}

==> tables/task_example.tex <==
\begin{table*}[t!]
    \centering
    \small
    
    \scalebox{0.85}{\begin{tabular}{l l}  \toprule %
    
    \textbf{Task} & \textbf{Example} \\\midrule
     
    Semantic-Graph & A \ModifierColor{tall} \NegationColor{boy} is \QuantifierColor{running} \ModifierColor{quickly} to catch a \ModifierColor{soccer} \NegationColor{ball}. \\[5pt]
    (SemGraph) & \NegationColor{[boy]} \QuantifierColor{[running]}  $\longrightarrow$ \textbf{Concept-Relation}; \ModifierColor{[tall]} \NegationColor{[boy]} $\longrightarrow$ \textbf{Concept-Modifier};\\[5pt] 
    & \ModifierColor{[quickly]} \QuantifierColor{[running]} $\longrightarrow$ \textbf{Relation-Modifier} \\[5pt] \midrule
    
    Monotonicity & Some$^\uparrow$ people$^\uparrow$ in$^\uparrow$ the$^\uparrow$ White$^=$ House$^=$ does$^\uparrow$ not$^\uparrow$ know$^\downarrow$ if$^\downarrow$ any$^\downarrow$ dog$^\downarrow$ in$^\downarrow$ Ohio$^\downarrow$ ate$^\downarrow$ bananas$^\downarrow$ yesterday$^\downarrow$ \\ \midrule
    
    Lexical & P: The \QuantifierColor{man} is holding a \ModifierColor{saxophone} \\ [5pt]
    (SA-Lex) & H: The man is holding an \ModifierColor{instrument}. \\ [5pt]
    & \QuantifierColor{[man]} \ModifierColor{[instrument]}  $\longrightarrow$ \textbf{Unaligned}; \ModifierColor{[saxophone]} \ModifierColor{[instrument]} $\longrightarrow$ \textbf{Aligned} \\ [5pt] \midrule
     
    Anaphora & The \QuantifierColor{technician} told the \ModifierColor{customer} that \ModifierColor{he} could pay with cash.  \\[5pt]
    (SA-AP) & \QuantifierColor{[technician]} \ModifierColor{[he]}  $\longrightarrow$ \textbf{Unaligned}; \ModifierColor{[customer]} \ModifierColor{[he]} $\longrightarrow$ \textbf{Aligned} \\ [5pt] \midrule
    
    Sentiment & P: When asked about the restaurant, Brielle said, ``\ModifierColor{It was terrible!} \QuantifierColor{I found this product to be way too big} '' \\[5pt]
    (SA-ST) & H: Brielle \ModifierColor{did not like the restaurant}  \\[5pt]
    & \QuantifierColor{[I found this product to be way too big]} \ModifierColor{[did not like the restaurant]} $\longrightarrow$ \textbf{Unaligned}\\  [5pt] 
    & \ModifierColor{[It was terrible]} \ModifierColor{[did not like the restaurant]} $\longrightarrow$ \textbf{Aligned} \\ [5pt] \midrule
    
    Relational-Knowledge & P: \ModifierColor{Dirk Nowitski is a current NBA star} playing with the \QuantifierColor{Dallas Mavericks as an all-purpose forward} \\[5pt]
    (SA-RK) & H: \ModifierColor{Dirk Nowitski plays in the NBA} \\[5pt] 
    & \QuantifierColor{[Dallas Mavericks as an all-purpose forward]} \ModifierColor{[Dirk Nowitski plays in the NBA]} $\longrightarrow$ \textbf{Unaligned} \\ [5pt] 
    & \ModifierColor{[Dirk Nowitski is a current NBA star]} \ModifierColor{[Dirk Nowitski plays in the NBA]} $\longrightarrow$ \textbf{Aligned} \\ [5pt]  \midrule
    
    Contradiction Signature & P: Italy and Germany \QuantifierColor{have each played twice}, and they \NegationColor{haven't beaten anybody yet} \\[5pt]
     (ContraSig) & H: Italy \NegationColor{defeats Germany} \\[5pt]
     & \QuantifierColor{[have each played twice]} \NegationColor{[defeats Germany]} $\longrightarrow$ \textbf{None} \\ [5pt] 
     & \NegationColor{[haven't beaten anybody yet]} \NegationColor{[defeats Germany]} $\longrightarrow$ \textbf{Contra-sig} \\ [5pt] 
      
      \bottomrule
      \end{tabular}}
      \caption{\small This table lists examples for the semantic alignment tasks and the contradiction signature detection task. The red boxes are spans that are semantically aligned. The yellow boxes are spans that form a contradiction signature. The blue boxes are spans that are irrelevant to semantic alignment or contradiction. Here P stands for a premise, and H stands for a hypothesis. The anaphora-based alignment only uses a single sentence. For the labels, ($s^1, s^3$) $\longrightarrow$ \textbf{Aligned} means that $s^1$ and $s^3$ are aligned. \{$t^1$, $\dots$, $t^7$\} $\longrightarrow$ \textbf{Align}$_1$ means that tokens $t^1$ to $t^7$ belongs to the first phrase in a semantically aligned pair.}
    \label{tab:data_exp}
\end{table*}
